RAMP: A Benchmark for Evaluating Robotic Assembly Manipulation and Planning

We introduce RAMP, an open-source robotics benchmark inspired by real-world industrial assembly tasks. RAMP consists of beams that a robot must assemble into specified goal configurations using pegs as fasteners. As such, it assesses planning and execution capabilities, and poses challenges in perception, reasoning, manipulation, diagnostics, fault recovery, and goal parsing. RAMP has been designed to be accessible and extensible. Parts are either 3D printed or otherwise constructed from materials that are readily obtainable. The design of parts and detailed instructions are publicly available. In order to broaden community engagement, RAMP incorporates fixtures such as April Tags which enable researchers to focus on individual sub-tasks of the assembly challenge if desired. We provide a full digital twin as well as rudimentary baselines to enable rapid progress. Our vision is for RAMP to form the substrate for a community-driven endeavour that evolves as capability matures.

==> old_bbl.tex <==
% Generated by IEEEtran.bst, version: 1.14 (2015/08/26)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{manyika2017future}
J.~Manyika, M.~Chui, M.~Miremadi, J.~Bughin, K.~George, P.~Willmott, and
  M.~Dewhurst, ``A future that works: Ai, automation, employment, and
  productivity,'' \emph{McKinsey Global Institute Research, Tech. Rep},
  vol.~60, pp. 1--135, 2017.

\bibitem{smith2016off}
R.~E. Smith, ``Off-site and modular construction explained,'' \emph{National
  institute of building sciences}, 2016.

\bibitem{OffsiteConstruction}
R.~H. Assaad, I.~H. El-adaway, M.~Hastak, and K.~L. Needy, ``Quantification of
  the state of practice of offsite construction and related technologies:
  Current trends and future prospects,'' \emph{Journal of Construction
  Engineering and Management}, vol. 148, no.~7, p. 04022055, 2022.

\bibitem{Krizhevsky2012ImagenetNetworks}
A.~Krizhevsky, I.~Sutskever, and G.~E. Hinton, ``{Imagenet classification with
  deep convolutional neural networks},'' \emph{Advances in neural information
  processing systems}, vol.~25, pp. 1097--1105, 2012.

\bibitem{Geiger2012}
A.~Geiger, P.~Lenz, and R.~Urtasun, ``{Are we ready for autonomous driving? The
  KITTI vision benchmark suite},'' in \emph{2012 IEEE Conference on Computer
  Vision and Pattern Recognition}, 2012, pp. 3354--3361.

\bibitem{OpenAIGym}
G.~Brockman, V.~Cheung, L.~Pettersson, J.~Schneider, J.~Schulman, J.~Tang, and
  W.~Zaremba, ``Openai gym,'' 2016.

\bibitem{IsaacDeveloper}
\BIBentryALTinterwordspacing
NVIDIA, ``Nvidia isaac sim.'' [Online]. Available:
  \url{https://developer.nvidia.com/isaac-sim}
\BIBentrySTDinterwordspacing

\bibitem{Calli2015BenchmarkingSet}
B.~Calli, A.~Walsman, A.~Singh, S.~Srinivasa, P.~Abbeel, and A.~M. Dollar,
  ``{Benchmarking in Manipulation Research: Using the Yale-CMU-Berkeley Object
  and Model Set},'' \emph{IEEE Robotics {\&} Automation Magazine}, vol.~22,
  no.~3, pp. 36--52, 2015.

\bibitem{Mnyusiwalla2020ASystems}
H.~Mnyusiwalla, P.~Triantafyllou, P.~Sotiropoulos, M.~A. Roa, W.~Friedl, A.~M.
  Sundaram, D.~Russell, and G.~Deacon, ``{A Bin-Picking Benchmark for
  Systematic Evaluation of Robotic Pick-and-Place Systems},'' \emph{IEEE
  Robotics and Automation Letters}, vol.~5, no.~2, pp. 1389--1396, 2020.

\bibitem{Garcia-Camacho2020BenchmarkingManipulation}
I.~Garcia-Camacho, M.~Lippi, M.~C. Welle, H.~Yin, R.~Antonova, A.~Varava,
  J.~Borras, C.~Torras, A.~Marino, G.~Aleny{\`{a}}, and D.~Kragic,
  ``{Benchmarking Bimanual Cloth Manipulation},'' \emph{IEEE Robotics and
  Automation Letters}, vol.~5, no.~2, pp. 1111--1118, 2020.

\bibitem{Collins2019BenchmarkingDataset}
J.~Collins, J.~McVicar, D.~Wedlock, R.~Brown, D.~Howard, and J.~Leitner,
  ``{Benchmarking Simulated Robotic Manipulation through a Real World
  Dataset},'' \emph{IEEE Robotics and Automation Letters}, 2019.

\bibitem{Suarez2020BenchmarksManipulation}
A.~Suarez, V.~M. Vega, M.~Fernandez, G.~Heredia, and A.~Ollero, ``{Benchmarks
  for Aerial Manipulation},'' \emph{IEEE Robotics and Automation Letters},
  vol.~5, no.~2, pp. 2650--2657, 2020.

\bibitem{JIANG2022102366}
Y.~Jiang, Z.~Huang, B.~Yang, and W.~Yang, ``A review of robotic assembly
  strategies for the full operation procedure: planning, execution and
  evaluation,'' \emph{Robotics and Computer-Integrated Manufacturing}, vol.~78,
  p. 102366, 2022.

\bibitem{yu2019meta}
T.~Yu, D.~Quillen, Z.~He, R.~Julian, K.~Hausman, C.~Finn, and S.~Levine,
  ``Meta-world: A benchmark and evaluation for multi-task and meta
  reinforcement learning,'' in \emph{Conference on Robot Learning (CoRL)},
  2019.

\bibitem{SURREAL}
L.~Fan, Y.~Zhu, J.~Zhu, Z.~Liu, O.~Zeng, A.~Gupta, J.~Creus-Costa, S.~Savarese,
  and L.~Fei-Fei, ``Surreal: Open-source reinforcement learning framework and
  robot manipulation benchmark,'' in \emph{Proceedings of The 2nd Conference on
  Robot Learning}, ser. Proceedings of Machine Learning Research,
  vol.~87.\hskip 1em plus 0.5em minus 0.4em\relax PMLR, 29--31 Oct 2018, pp.
  767--782.

\bibitem{Lee2021IKEATasks}
Y.~Lee, E.~S. Hu, and J.~J. Lim, ``{IKEA Furniture Assembly Environment for
  Long-Horizon Complex Manipulation Tasks},'' in \emph{2021 IEEE International
  Conference on Robotics and Automation (ICRA)}, 2021, pp. 6343--6349.

\bibitem{Yichen}
Y.~Li, K.~Mo, L.~Shao, M.~Sung, and L.~Guibas, ``Learning 3d part assembly from
  a single image,'' in \emph{Computer Vision -- ECCV 2020}.\hskip 1em plus
  0.5em minus 0.4em\relax Cham: Springer International Publishing, 2020, pp.
  664--682.

\bibitem{Kimble2020BenchmarkingSystems}
K.~Kimble, J.~Falco, E.~Messina, K.~V. Wyk, Y.~Sun, M.~Shibata, W.~Uemura, and
  Y.~Yokokohji, ``\BIBforeignlanguage{en}{{Benchmarking Protocols for
  Evaluating Small Parts Robotic Assembly Systems}},'' 2020.

\bibitem{Chatzilygeroudis2020BenchmarkObjects}
K.~Chatzilygeroudis, B.~Fichera, I.~Lauzana, F.~Bu, K.~Yao, F.~Khadivar, and
  A.~Billard, ``{Benchmark for Bimanual Robotic Manipulation of Semi-Deformable
  Objects},'' \emph{IEEE Robotics and Automation Letters}, vol.~5, no.~2, pp.
  2443--2450, 2020.

\bibitem{Spector}
O.~Spector and D.~D. Castro, ``Insertionnet - a scalable solution for
  insertion,'' \emph{IEEE Robotics and Automation Letters}, vol.~6, no.~3, pp.
  5509--5516, 2021.

\bibitem{LegoBot}
L.~Nägele, A.~Hoffmann, A.~Schierl, and W.~Reif, ``Legobot: Automated planning
  for coordinated multi-robot assembly of lego structures,'' in \emph{2020
  IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  2020, pp. 9088--9095.

\bibitem{Ghasemipour2022BlocksLearning}
S.~K.~S. Ghasemipour, D.~Freeman, B.~David, S.~S. Gu, S.~Kataoka, and
  I.~Mordatch, ``{Blocks Assemble! Learning to Assemble with Large-Scale
  Structured Reinforcement Learning},'' 3 2022.

\bibitem{Suarez-Ruiz2018CanChair}
F.~Su{\'{a}}rez-Ruiz, X.~Zhou, and Q.-C. Pham, ``{Can robots assemble an IKEA
  chair?}'' \emph{Science Robotics}, vol.~3, no.~17, p. eaat6385, 4 2018.

\bibitem{Knepper2013IkeaBot:System}
R.~A. Knepper, T.~Layton, J.~Romanishin, and D.~Rus, ``{IkeaBot: An autonomous
  multi-robot coordinated furniture assembly system},'' in \emph{2013 IEEE
  International Conference on Robotics and Automation}, 2013, pp. 855--862.

\bibitem{Thoma2019RoboticModules}
A.~Thoma, A.~Adel, M.~Helmreich, T.~Wehrle, F.~Gramazio, and M.~Kohler,
  ``{Robotic Fabrication of Bespoke Timber Frame Modules},'' \emph{Robotic
  Fabrication in Architecture, Art and Design 2018}, pp. 447--458, 2019.

\bibitem{CARA}
H.~Fakhurldeen, F.~Dailami, and A.~G. Pipe, ``Cara system architecture - a
  click and assemble robotic assembly system,'' in \emph{2019 International
  Conference on Robotics and Automation (ICRA)}, 2019, pp. 5830--5836.

\bibitem{Zobov2023Auto-Assembly:CAD}
S.~Zobov, F.~Chervinskii, A.~Rybnikov, D.~Petrov, and K.~Vendidandi,
  ``{Auto-Assembly: a framework for automated robotic assembly directly from
  CAD},'' 1 2023.

\bibitem{FetchitChallenge}
\BIBentryALTinterwordspacing
``{Fetchit! The Mobile Manipulation Challenge}.'' [Online]. Available:
  \url{https://opensource.fetchrobotics.com/competition}
\BIBentrySTDinterwordspacing

\bibitem{Yokokohji2019Assembly2018}
Y.~Yokokohji, Y.~Kawai, M.~Shibata, Y.~Aiyama, S.~Kotosaka, W.~Uemura, A.~Noda,
  H.~Dobashi, T.~Sakaguchi, and K.~Yokoi, ``{Assembly Challenge: a robot
  competition of the Industrial Robotics Category, World Robot Summit –
  summary of the pre-competition in 2018},'' \emph{Advanced Robotics}, vol.~33,
  no.~17, pp. 876--899, 9 2019.

\bibitem{nist_2022}
\BIBentryALTinterwordspacing
``Icra 2022 robotic grasping and manipulation competition: Manufacturing
  track,'' Apr 2022. [Online]. Available:
  \url{https://www.nist.gov/el/intelligent-systems-division-73500/icra-2022-robotic-grasping-and-manipulation-competition}
\BIBentrySTDinterwordspacing

\bibitem{Olson2011AprilTag:System}
E.~Olson, ``{AprilTag: A robust and flexible visual fiducial system},'' in
  \emph{2011 IEEE International Conference on Robotics and Automation}, 2011,
  pp. 3400--3407.

\bibitem{Macklin2020LocalCollision}
M.~Macklin, K.~Erleben, M.~M{\"{u}}ller, N.~Chentanez, S.~Jeschke, and
  Z.~Corse, ``{Local Optimization for Robust Signed Distance Field Coll
  ision},'' \emph{Proc. ACM Comput. Graph. Interact. Tech.}, vol.~3, no.~1, 5
  2020.

\bibitem{Sridharan2019REBA}
M.~Sridharan, M.~Gelfond, S.~Zhang, and J.~L. Wyatt, ``{REBA:} {A}
  refinement-based architecture for knowledge representation and reasoning in
  robotics,'' \emph{J. Artif. Intell. Res.}, vol.~65, pp. 87--180, 2019.

\bibitem{Gelfond2013ALD}
M.~Gelfond and D.~Inclezan, ``Some properties of system descriptions of ald,''
  \emph{Journal of Applied Non-Classical Logics}, vol.~23, no. 1-2, pp.
  105--120, 2013.

\bibitem{gelfond2014ASP}
M.~Gelfond and Y.~Kahl, \emph{Knowledge Representation, Reasoning, and the
  Design of Intelligent Agents: The Answer-Set Programming Approach}.\hskip 1em
  plus 0.5em minus 0.4em\relax Cambridge University Press, 2014.

\bibitem{Balai2013SPARC}
E.~Balai, M.~Gelfond, and Y.~Zhang, ``{SPARC} - sorted {ASP} with consistency
  restoring rules,'' \emph{CoRR}, vol. abs/1301.1386, 2013.

\bibitem{Gebser2019MultishotASPSWC}
M.~Gebser, R.~Kaminski, B.~Kaufmann, and T.~Schaub, ``Multi-shot asp solving
  with clingo,'' \emph{TPLP}, vol.~19, p. 27–82, 2019.

\bibitem{gorner2019moveit}
M.~G{\"o}rner, R.~Haschke, H.~Ritter, and J.~Zhang, ``Moveit! task constructor
  for task-level motion planning,'' in \emph{2019 International Conference on
  Robotics and Automation (ICRA)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE,
  2019, pp. 190--196.

\bibitem{chhatpar2001search}
S.~Chhatpar and M.~Branicky, ``Search strategies for peg-in-hole assemblies
  with position uncertainty,'' in \emph{Proceedings 2001 IEEE/RSJ International
  Conference on Intelligent Robots and Systems.}, vol.~3, 2001.

\bibitem{garrett:ARCRAS21}
C.~R. Garrett, R.~Chitnis, R.~Holladay, B.~Kim, T.~Silver, L.~P. Kaelbling, and
  T.~Lozano-Perez, ``{Integrated Task and Motion Planning},'' \emph{Annual
  Review of Control, Robotics, and Autonomous Systems}, vol.~4, pp. 265--293,
  2021.

\bibitem{yamada2023leveraging}
J.~Yamada, C.-M. Hung, J.~Collins, I.~Havoutis, and I.~Posner, ``Leveraging
  scene embeddings for gradient-based motion planning in latent space,'' in
  \emph{2023 IEEE International Conference on Robotics and Automation
  (ICRA)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2023.

\bibitem{yamada2023efficient}
J.~Yamada, J.~Collins, and I.~Posner, ``Efficient skill acquisition for complex
  manipulation tasks in obstructed environments,'' \emph{arXiv preprint
  arXiv:2303.03365}, 2023.

\bibitem{yamada2020mopa}
J.~Yamada, Y.~Lee, G.~Salhotra, K.~Pertsch, M.~Pflueger, G.~S. Sukhatme, J.~J.
  Lim, and P.~Englert, ``Motion planner augmented reinforcement learning for
  obstructed environments,'' in \emph{Conference on Robot Learning}, 2020.

\bibitem{Lambeta_2020}
M.~Lambeta, P.-W. Chou, S.~Tian, B.~Yang, B.~Maloon, V.~R. Most, D.~Stroud,
  R.~Santos, A.~Byagowi, G.~Kammerer, D.~Jayaraman, and R.~Calandra, ``{DIGIT}:
  A novel design for a low-cost compact high-resolution tactile sensor with
  application to in-hand manipulation,'' \emph{{IEEE} Robotics and Automation
  Letters}, vol.~5, no.~3, pp. 3838--3845, jul 2020.

\bibitem{AssembleThemAll}
Y.~Tian, J.~Xu, Y.~Li, J.~Luo, S.~Sueda, H.~Li, K.~D.~D. Willis, and
  W.~Matusik, ``Assemble them all: Physics-based planning for generalizable
  assembly by disassembly,'' vol.~41, no.~6, 2022.

\end{thebibliography}

